A Parallel Sparse Tensor Benchmark Suite on CPUs and GPUs

Tensor computations present significant performance challenges that impact a wide spectrum of applications ranging from machine learning, healthcare analytics, social network analysis, data mining to quantum chemistry and signal processing. Efforts to improve the performance of tensor computations include exploring data layout, execution scheduling, and parallelism in common tensor kernels. This work presents a benchmark suite for arbitrary-order sparse tensor kernels using state-of-the-art tensor formats: coordinate (COO) and hierarchical coordinate (HiCOO) on CPUs and GPUs. It presents a set of reference tensor kernel implementations that are compatible with real-world tensors and power law tensors extended from synthetic graph generation techniques. We also propose Roofline performance models for these kernels to provide insights of computer platforms from sparse tensor view.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-sigconf.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> src/algs/alg-coo-mttkrp.tex <==

\begin{algorithm}[h]
\footnotesize
\caption{COO-\MTTKRP-OMP algorithm in mode-1 \cite{Bader:2007:tensortoolbox-sparse}.}
\begin{algorithmic}[1]
  \Require
       A third-order sparse tensor $\T{X} \in \R^{I \times J \times K}$ with \nnz non-zeros in COO format, dense matrices $\M{B} \in \R^{J \times R}, \M{C} \in \R^{K \times R}$;
  \Ensure
       Updated dense matrix $\tilde{\M{A}} \in \R^{I \times R}$;

  \Statex \Comment{$\tilde{\M{A}} \leftarrow \T{X}_{(1)} (\M{C} \odot \M{B})$} 

  \PARFOR{$m=1, \dots, \nnz$}
  % \Comment{Parallelize}
  % \For{$m=1, \dots, \nnz$}
  	\State $i = \inds^1(m)$, $j = \inds^2(m)$, $k = \inds^3(m)$
    % \Statex \Comment{Continuous RD -> Reg}
    \State $value = \val(m)$
    % \Comment{Continuous RD -> Reg}
  	\For{$r=1, \dots, R$}
  		\State  $\tilde{A}(i \times R + r) += value \times C(k \times R + r) \times B(j \times R + r)$
      % \Statex \Comment{Continuous RD -> Continuous WR}
  	\EndFor
  % \EndFor \\
  \ENDPARFOR

  % \Return{} $\tilde{\M{A}}$;
  \State \textbf{Return} $\tilde{\M{A}}$;
\end{algorithmic}
\label{alg:mttkrp}
\end{algorithm}


==> src/algs/alg-coo-tew-eq.tex <==

\begin{algorithm}[h]
\small
\caption{Sequential COO-\TEW-eq-Add algorithm for tensors in the same order and shape.}
\begin{algorithmic}[1]
  \Require
       A third-order sparse tensor $\T{X}, \T{Y} \in \R^{I \times J \times K}$ with $\nnz$ non-zeros;
  \Ensure
       Sparse tensor $\T{Z} \in \R^{I \times J \times K}$;

  \Statex \Comment{$\T{Z} = \T{X} .+ \T{Y}$} 

  \State Allocate \T{Z} space with $\nnz$ non-zeros; \Comment{Pre-allocation space.}

  \For{$m=1, \dots, \nnz$}
  	\State $\val_z(m) = \val_x(m) + \val_y(m)$;
  \EndFor \\
  \Return{} $\T{Z}$;
\end{algorithmic}
\label{alg:tew-eq}
\end{algorithm}


==> src/algs/alg-coo-tew.tex <==
\begin{algorithm}[h]
\small
\caption{Sequential COO-\TEW-Addition algorithm for general tensors.}
\begin{algorithmic}[1]
  \Require
       A third-order sparse tensor $\T{X} \in \R^{I_1 \times J_1 \times K_1}$ with $\nnz_1$ non-zeros, $\T{Y} \in \R^{I_2 \times J_2 \times K_2}$ with $\nnz_2$ non-zeros;
  \Ensure
       Sparse tensor $\T{Z} \in \R^{I_3 \times J_3 \times K_3}$;

  \Statex \Comment{$\T{Z} = \T{X} .+ \T{Y}$} 

  \State $I_3 = max\{I_1, I_2\}$, $J_3 = max\{J_1, J_2\}$, $K_3 = max\{K_1, K_2\}$ \Comment{Unify the tensor shape.}

  \State Sort \T{X} and \T{Y} in the same dimension order.

  \State $m_1=1$, $m_2=1$
  \While{$m_1<\nnz_1$ and $m_2<\nnz_2$}
  	\If{$\inds_x == \inds_y$}
  		\State Append($\inds^1_z$, $\inds^1_x(m_1)$); Append($\inds^2_z$, $\inds^2_x(m_1)$); Append($\inds^3_z$, $\inds^3_x(m_1)$);
  		\State Append($\val_z$, $\val_x(m_1) + \val_y(m_2)$);
	\EndIf
  	\If{$\inds_x > \inds_y$}
  		\State Append($\inds^1_z$, $\inds^1_y(m_1)$); Append($\inds^2_z$, $\inds^2_y(m_1)$); Append($\inds^3_z$, $\inds^3_y(m_1)$);
  		\State Append($\val_z$, $\val_y(m_2)$);
  	\EndIf
  	\If{$\inds_x < \inds_y$}
  		\State Append($\inds^1_z$, $\inds^1_x(m_1)$); Append($\inds^2_z$, $\inds^2_x(m_1)$); Append($\inds^3_z$, $\inds^3_x(m_1)$);
  		\State Append($\val_z$, $\val_x(m_1)$);
  	\EndIf
  \EndWhile 
  \If{$m_1 < \nnz_1$}
  	\State Append($\inds^1_z$, $\inds^1_x(m_1,:)$); Append($\inds^2_z$, $\inds^2_x(m_1,:)$); Append($\inds^3_z$, $\inds^3_x(m_1,:)$);
  	\State Append($\val_z$, $\val_x(m_1,:)$)
  \EndIf
  \If{$m_2 < \nnz_2$}
  	\State Append($\inds^1_z$, $\inds^1_x(m_2,:)$); Append($\inds^2_z$, $\inds^2_x(m_2,:)$); Append($\inds^3_z$, $\inds^3_x(m_2,:)$);
  	\State Append($\val_z$, $\val_x(m_2,:)$)
  \EndIf
  \\
  \Return{} $\T{Z}$;
\end{algorithmic}
\label{alg:tew}
\end{algorithm}


==> src/algs/alg-coo-ts.tex <==

\begin{algorithm}[h]
\small
\caption{Sequential COO-\TSM algorithm.}
\begin{algorithmic}[1]
  \Require
       A third-order sparse tensor $\T{X} \in \R^{I \times J \times K}$ with $\nnz$ non-zeros;
  \Ensure
       Output sparse tensor $\T{Y} \in \R^{I \times J \times K}$;

  \Statex \Comment{$\T{Y} = \T{X} \times s$} 

  \State Allocate \T{Y} space with $\nnz$ non-zeros; \Comment{Pre-allocation space.}

  \For{$m=1, \dots, \nnz$}
  	\State $\inds^1_y(m) = \inds^1_x(m)$, $\inds^2_y(m) = \inds^2_x(m)$, $\inds^3_y(m) = \inds^3_x(m)$;
  	\State $\val_y(m) = s \times \val_x(m)$;
  \EndFor \\
  \Return{} $\T{Y}$;
\end{algorithmic}
\label{alg:ts}
\end{algorithm}


==> src/algs/alg-coo-ttm.tex <==
\begin{algorithm}[ht]
\footnotesize
\caption{COO-\TTM-OMP algorithm~\cite{Li:2016:spttm}.}
\begin{algorithmic}[1]
  \Require
       A sparse tensor $\T{X} \in \R^{I \times J \times K}$ with \nnz non-zeros in COO format, a dense matrix $\M{U} \in \R^{K \times R}$, and an integer $n$($=3$);
  \Ensure
       A semi-sparse tensor $\T{Y} \in \R^{I \times J \times R}$ in sCOO format;
  \Statex \Comment{$\T{Y} = \T{X} \times_n \M{U}$}

  \State Pre-process to obtain $\nfibs$, the number of mode-n fibers of \T{X} and $\fptr$, the beginnings of each \T{X} mode-n fiber, size $\nfibs$.
  \State Pre-allocate \T{Y} space with $\nfibs \times R$ non-zeros and their indices; 
  \Statex

  \PARFOR{$f=1, \dots, \nfibs$}
  % \Comment{Parallelize}
  % \For{$f=1, \dots, \nfibs$}
    \State $f_X = \fptr(f)$
    % \Comment{Continuous RD -> Reg}
    % \State $\inds^1_Y(f) = \inds^1_X(f_X)$
    % \Comment{Strided RD -> Continuous WR}
    % \State $\inds^2_Y(f) = \inds^2_X(f_X)$
    % \Comment{Strided RD -> Continuous WR}
    \State $vec = \val_Y + f \times R$
    % \Comment{Save a pointer.}

    \For{$m=f_X, \dots, \fptr(f+1)-1$}
      \State $k = \inds^n_X(m)$
      % \Comment{Continuous RD -> Reg}
      \State $value = \val_X(m)$
      % \Comment{Continuous RD -> Reg}
      \For{$r=1, \dots, R$}
        \State $vec(r) += value \times u(k \times R + r)$
        % \Statex \Comment{Continuous RD -> Continuous WR}
      \EndFor
    \EndFor
  % \EndFor
  \ENDPARFOR

  \State \textbf{Return} \T{Y};
\end{algorithmic}
\label{alg:ttm}
\end{algorithm}


==> src/algs/alg-hicoo-ttm.tex <==
\begin{algorithm}[h]
\footnotesize
\caption{CPU-Parallel HiCOO-\TTM algorithm in mode-1~\cite{Li:2018:hicoo}.}
\begin{algorithmic}[1]
\footnotesize
  \Require
       A sparse tensor $\T{X} \in \R^{I \times J \times K}$ with \nnz non-zeros in gHiCOO format, a dense matrix $\M{U} \in \R^{K \times R}$, block size $B$, and an integer $n$ ($=3$);
  \Ensure
       A semi-sparse tensor$\T{Y} \in \R^{I \times J \times R}$ in sHiCOO format;

  \Statex \Comment{$\T{Y} = \T{X} \times_n \M{U}$}

  \State Pre-process to obtain $\nfibs$, the number of mode-n fibers of \T{X} and $\fptr$, the beginnings of each \T{X} mode-n fiber, size $\nfibs$.
  \State Pre-allocate \T{Y} space with $\nfibs \times R$ non-zeros and their indices; 
  \Statex

  \PARFOR{$b=1, \dots, n_b$} \Comment{Parallelize block $b$}
    \State $bptr_Y(b) = bptr_X(b)$
    \Comment{Continuous RD -> Continuous WR}
    \State $\binds_Y^1(b) = \binds_X^1(b)$, $\binds_Y^2(b) = \binds_X^2(b)$;
    \Statex \Comment{Continuous RD -> Continuous WR}

    \Statex \Comment{Parallelize fiber $f$}
    \PARFOR{$f=bptr_X(b), \dots, bptr_X(b+1) - 1$}
      \State $\einds_Y^1(f) = \einds_X^1(f)$, $\einds_Y^2(f) = \einds^2(f)$
      \Statex \Comment{Continuous RD -> Continuous WR}

      \State $f_X = \fptr(f)$
      \Comment{Continuous RD -> Reg}
      \State $vec = \val_Y + f \times R$
      \Comment{Save a pointer.}

      % \PARFOR{$f=1, \dots, \nfibs$}
      % \Comment{Parallelize}
      % \For{$f=1, \dots, \nfibs$}
      \For{$m=f_X, \dots, \fptr(f+1)-1$}
        \State $k = \inds^n_X(m)$
        \Comment{Continuous RD -> Reg}
        \State $value = \val_X(m)$
        \Comment{Continuous RD -> Reg}
        \For{$r=1, \dots, R$}
          \State $vec(r) += value \times u(k \times R + r)$
          \Statex \Comment{Continuous RD -> Continuous WR}
        \EndFor
      \EndFor
    \ENDPARFOR
  \ENDPARFOR

  % \Return{} $\tilde{\M{A}}$;
  \State \textbf{Return} $\tilde{\M{A}}$;
\end{algorithmic}
\label{alg:mttkrp-hicoo}
\end{algorithm}


==> src/back.tex <==
  


==> src/tab-analysis.tex <==
\begin{table}[ht!]
\centering
\footnotesize
{
\caption{The analysis of kernel algorithms for third-order cubical tensors ($\T{X} \in \R^{I \times I \times I}$). We consider all input tensors with \nnz non-zero entries and $\nnz_F$ fibers, $I \ll \nfibs \ll \nnz$. The indices use $32$ bits, and values are single-precision floating-point numbers with $32$ bits as well.}
\label{tab:analysis}
\begin{tabular}{rcccc}
  % \hline
  \toprule
  
  Kernels & 
  % Storage (#\Bytes) & \multirow{2}{*}{AI}
  Work (\#Flops) & 
  Memory Access (\#Bytes)$^*$ & 
  Arithmetic Intensity \\ \hline

  \TEW & 
  % $48 \nnz $ & 
  $\nnz$ & 
  $12 \nnz$ &
  $1/12$ \\

  \TS & 
  % $32 \nnz $ & 
  $\nnz$ & 
  $8 \nnz$ &
  $1/8$ \\

  \TTV & 
  % $16 \nnz + 12 \nfibs + 4I $ & 
  $2 \nnz$ & 
  $8 \nnz + 4 \nfibs$ &
  $\sim 1/4$ \\

  \TTM & 
  % $16 \nnz + 16 \nfibs R + 4IR $ & 
  $2 \nnz R$ & 
  $4 \nnz R + 4 \nfibs R + 4 \nnz$ &
  $\sim 1/2$ \\

  \MTTKRP & 
  % $16 \nnz + 12 IR$ & 
  $3 \nnz R$ & 
  $12 \nnz R + 4 \nnz$ &
  $\sim 1/4$ \\

  \bottomrule
\end{tabular}
\\ $^*$ \footnotesize{The memory access considers only that of floating-point values. We leave the indices pattern for memory access to calculate the performance upper-bound and being able to compare between implementations for different formats and tensor orders. \rv{Cache effect is not considered because of the irregular memory access inside.}}
}
% \\ $^1$ {\MTTKRP}s in all tensor modes can use less CSF representations than tensor order or even only one CSF representation with performance payoff.
\end{table}



==> src/tab-dataset.tex <==
\begin{table}[htbp]
\centering
\small
{
\caption{Description of sparse tensors.}
\label{tab:real-tensors}
\begin{tabular}{rcccc}
  Tensors & Order & Dimensions & \#Nnzs & Density \\
  \toprule
  % Real & & & \\ \cline{1-1}
  \tennm{vast} & 3 & $165K \times 11K \times 2$ & 26M & $6.9 \times 10^{-3}$ \\
  \tennm{nell2} & 3 & $12K \times 9K \times 29K$ & 77M & $2.4 \times 10^{-5}$ \\
  \tennm{choa} & 3 & $712K \times 10K \times 767$ & 27M & $5.0 \times 10^{-6}$ \\
  \tennm{darpa} & 3 & $22K \times 22K \times 24M$ & 28M & $2.4 \times 10^{-9}$ \\
  \tennm{fb-m} & 3 & $23M \times 23M \times 166$ & 100M & $1.1 \times 10^{-9}$ \\
  \tennm{fb-s} & 3 & $39M \times 39M \times 532$ & 140M & $1.7 \times 10^{-10}$ \\
  % \tennm{flickr} & 3 & $320K \times 28M \times 1.6M$ & 113M & $7.8 \times 10^{-12}$ \\
  \tennm{deli} & 3 & $533K \times 17M \times 2.5M$ & 140M & $6.1 \times 10^{-12}$ \\
  \tennm{nell1} & 3 & $2.9M \times 2.1M \times 25M$ & 144M & $9.1 \times 10^{-13}$ \\ 
  \midrule
  \tennm{crime4d} & 4 & $6K \times 24 \times 77 \times 32$ & 5M & $1.5 \times 10^{-2}$ \\
  % \tennm{uber} & 4 & $183 \times 24 \times 1140 \times 1717$ & 3M & $3.9 \times 10^{-4}$ \\
  \tennm{nips4d} & 4 & $2K \times 3K \times 14K \times 17$ & 3M & $1.8 \times 10^{-6}$ \\ 
  \tennm{enron4d} & 4 & $6K \times 6K \times 244K \times 1K$ & 54M & $5.5 \times 10^{-9}$ \\ 
  \tennm{flickr4d} & 4 & $320K \times 28M \times 1.6M \times 731$ & 113M & $1.1 \times 10^{-14}$ \\ 
  \tennm{deli4d} & 4 & $533K \times 17M \times 2.5M \times 1K$ & 140M & $4.3 \times 10^{-15}$ \\ 
  % \midrule
  % Synthetic & & & & \\ \cline{1-1}
  % \tennm{pos-syn1} & 3 & $10K \times 10K \times 10K$ & 100M & $1.0 \times 10^{-4}$ \\
  % \tennm{pos-syn2} & 3 & $40K \times 40K \times 40K$ & 128M & $2.0 \times 10^{-6}$ \\
  % \tennm{pos-syn2} & 3 & $50K \times 50K \times 50K$ & 125M & $1.0 \times 10^{-6}$ \\
  \bottomrule
\end{tabular}
}
\end{table}

==> src/tab-platform.tex <==
\begin{table}[htbp]
\centering
\scriptsize
{
\caption{Platform parameters.}
\label{tab:platform}
\begin{tabular}{rccccc}
  % \hline
  \toprule
  
  \multirow{2}{*}{\textbf{Parameters}} &
  \multicolumn{3}{c}{\textbf{Intel CPUs}} &
  \multicolumn{2}{c}{\textbf{NVIDIA GPUs}} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-6}

   & 
  % \textbf{Bluesky} & 
  \textbf{DGX-CPU} & 
  \textbf{Cori} & 
  \textbf{Wingtip} & 
  \textbf{DGX-1P} &
  \textbf{DGX-1V} \\ \midrule
  % \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-6}

  \multirow{2}{*}{Processor} &
  % Intel Xeon &
  Intel Xeon &
  Intel Xeon &
  Intel Xeon &
  % AMD &
  NVIDIA &
  NVIDIA \\

   &
  % Gold 6126 &
  E5-2698v4 &
  E5-2698v3 &
  E7-4850v3 &
  % A10-7850K &
  Tesla P100 &
  Tesla V100 \\

  Microarch &
  % Skylake &
  Broadwell &
  Haswell &
  Haswell &
  % \al{TODO} &
  Pascal &
  Volta \\

  Frequency &
  % 2.60 GHz &
  2.20 GHz &
  2.30 GHz &
  2.20 GHz &
  % 3.70 GHz &
  1.48 GHz &
  1.53 GHz \\

  \#Cores &
  % 24 ($12 \times 2$) &
  40 ($20 \times 2$) &
  32 ($16 \times 2$) &
  56 ($14 \times 4$) &
  % 4 &
  3584 &
  5120 \\

  Peak SP perf. &
  % 1.0 TFLOPS &
  1.4 TFLOPS &
  1.2 TFLOPS &
  2.0 TFLOPS &
  % \al{TODO} &
  10.6 TFLOPS &
  14.9 TFLOPS \\

  LLC size &
  % 19 MB &
  50 MB &
  40 MB &
  35 MB &
  % 4 MB &
  3 MB &
  6 MB \\

  Mem. size &
  % 196 GB &
  528 GB &
  128 GB &
  2114 GB &
  % 32 GB &
  16 GB &
  16 GB \\

  Mem. type &
  % DDR4 &
  DDR4 &
  DDR4 &
  DDR4 &
   % &
  HBM2 &
  HBM2 \\

  Mem. freq. &
  % 2.666 GHz &
  2.133 GHz &
  2.133 GHz &
  2.133 GHz &
   % &
  0.715 GHz &
  0.877 GHz \\

  Mem. BW &
  % 256 GB/s &
  137 GB/s &
  137 GB/s &
  273 GB/s &
  % xx GB/s &
  732 GB/s &
  900 GB/s \\

  Compiler &
  % icc 17.0.4 &
  gcc 5.4.0 &
  icc 18.0.1 &
  gcc 5.5.0 &
  % gcc 4.8.5 &
  CUDA Tkit 9.1 &
  CUDA Tkit 9.0 \\

  \bottomrule
\end{tabular}
}
\end{table}



==> src/tab-storage.tex <==
\begin{table}[htbp]
\centering
\footnotesize
{
\caption{Sparse tensors memory storage.}
\label{tab:storage}
\begin{tabular}{cc}
  \begin{tabular}{rcc}
    Tensors & COO (MB) & HiCOO (MB) \\
    \toprule
    \tennm{vast} & 397 & 175 \\
    \tennm{nell2} & 1150 & 543 \\ 
    \tennm{choa} & 411 & 192 \\
    \tennm{darpa} & 434 & 307 \\ 
    \tennm{fb-m} & 1480 & 1420 \\ 
    \tennm{fb-s} & 2080 & 2110 \\
    \tennm{deli} & 2090 & 3490 \\
    \tennm{nell1} & 2140 & 3160 \\ 
    \midrule
    \tennm{crime4d} & 102 & 41 \\
    \tennm{nips4d} & 59 & 25 \\ 
    \tennm{enron4d} & 1010 & 459 \\ 
    \tennm{flickr4d} & 2100 & 1740 \\ 
    \tennm{deli4d} & 2610 & 3540 \\ 
    \bottomrule
  \end{tabular}

  \begin{tabular}{rcc}
    \multirow{2}{*}{Tensors} & \multirow{2}{*}{COO (MB)} & \multirow{2}{*}{HiCOO (MB)} \\
    & & \\
    \toprule
    \tennm{regS} & 16 & 25 \\
    \tennm{regM} & 175 & 293 \\
    \tennm{regL} & 1410 & 2380 \\
    \tennm{irrS} & 16 & 7 \\
    \tennm{irrM} & 156 & 70 \\
    \tennm{irrL} & 1260 & 584 \\
    \midrule
    \tennm{regS4d} & 19 & 25 \\
    \tennm{regM4d} & 215 & 344 \\
    \tennm{regL4d} & 2060 & 3290 \\
    \tennm{irrS4d} & 31 & 12 \\
    \tennm{irrM4d} & 373 & 149 \\
    \tennm{irrL4d} & 2030 & 833 \\
    \bottomrule
  \end{tabular}
\end{tabular}
}
\end{table}

==> src/tab-synthetic-ds.tex <==
\begin{table}[tb]
\centering
\footnotesize
\caption{Description of synthetic tensors generated (Gen.) with Kronecker and Power law generators indicated as Kron. and PL respectively.}
\label{tab:syn-tensors}
\begin{tabular}{rccccc}
\textbf{Tensors} & \textbf{Gen.} & \textbf{Order} & \textbf{Dimensions} & \textbf{\#Nnzs} & \textbf{Density} \\
\toprule
\tennm{regS} & Kron. & 3 & $(65K)^3$ & 1.1M & $3.72 \times 10^{-9}$ \\
\tennm{regM} & Kron. & 3 & $(1.1M)^3$ & 11.5M  & $9.97 \times 10^{-12}$ \\
\tennm{regL} & Kron. & 3 & $(8.3M)^3$  & 94M   & $1.61 \times 10^{-13}$  \\
\tennm{irrS} & PL & 3 & $(32K)^2 \times 76 $ & 1M & $1.26 \times 10^{-5}$ \\
\tennm{irrM} & PL & 3 & $(524K)^2 \times 126$ & 10M & $1.43 \times 10^{-6}$ \\
\tennm{irrL} & PL & 3 & $(4.2M)^2 \times 168$ & 84M & $2.86 \times 10^{-8}$ \\
\midrule
\tennm{regS4d} & Kron. & 4 & $(8.2K)^4$ & 1M & $2.26 \times 10^{-10}$ \\
\tennm{regM4d} & Kron. & 4 & $(2.1M^4)$ & 11.2M & $5.83 \times 10^{-19}$ \\
\tennm{regL4d} & Kron. & 4 & $(8.3M)^4$ & 110M & $2.23 \times 10^{-20}$ \\
\tennm{irrS4d} & PL & 4 & $(1.04M)^2 \times 122 \times 436$ & 1.6M & $2.81 \times 10^{-11}$ \\
\tennm{irrM4d} & PL & 4 & $(4.2M)^2 \times 232 \times 746$ & 19.9M & $6.53 \times 10^{-12}$ \\
\tennm{irrL4d} & PL & 4 & $(8.3M)^2 \times 952 \times 324$ & 109M  & $5.1\times 10^{-12}$ \\
\bottomrule
\end{tabular}
\end{table}


==> src/tabs/tab-analysis.tex <==
\begin{table}[ht!]
\centering
\footnotesize
{
\caption{The analysis of kernel algorithms for third-order cubical tensors ($\T{X} \in \R^{I \times I \times I}$). We consider all input tensors with \nnz non-zero entries and $\nnz_F$ fibers, $I \ll \nfibs \ll \nnz$. The indices use $32$ bits, and values are single-precision floating-point numbers with $32$ bits as well.}
\label{tab:analysis}
\begin{tabular}{rcccc}
  % \hline
  \toprule
  
  Kernels & 
  % Storage (#\Bytes) & \multirow{2}{*}{AI}
  Work (\#Flops) & 
  Memory Access (\#Bytes)$^*$ & 
  Operational Intensity \\ \hline

  \TEW & 
  % $48 \nnz $ & 
  $\nnz$ & 
  $12 \nnz$ &
  $1/12$ \\

  \TS & 
  % $32 \nnz $ & 
  $\nnz$ & 
  $8 \nnz$ &
  $1/8$ \\

  \TTV & 
  % $16 \nnz + 12 \nfibs + 4I $ & 
  $2 \nnz$ & 
  $8 \nnz + 4 \nfibs$ &
  $\sim 1/4$ \\

  \TTM & 
  % $16 \nnz + 16 \nfibs R + 4IR $ & 
  $2 \nnz R$ & 
  $4 \nnz R + 4 \nfibs R + 4 \nnz$ &
  $\sim 1/2$ \\

  \MTTKRP & 
  % $16 \nnz + 12 IR$ & 
  $3 \nnz R$ & 
  $12 \nnz R + 4 \nnz$ &
  $\sim 1/4$ \\

  \bottomrule
\end{tabular}
\\ $^*$ \footnotesize{The memory access considers only that of floating-point values. We leave the indices pattern for memory access to calculate the performance upper-bound and being able to compare between implementations for different formats and tensor orders. \rv{Cache effect is not considered because of the irregular memory access inside.}}
}
% \\ $^1$ {\MTTKRP}s in all tensor modes can use less CSF representations than tensor order or even only one CSF representation with performance payoff.
\end{table}



==> src/tabs/tab-full-analysis.tex <==
\begin{table*}[ht!]
\centering
\footnotesize
{
\caption{The analysis of kernel algorithms for third-order cubical tensors ($\T{X} \in \R^{I \times I \times I}$). We consider all input tensors with \nnz non-zero entries and $\nnz_F$ fibers, $I \ll \nfibs \ll \nnz$. The indices use $32$ bits, and values are single-precision floating-point numbers with $32$ bits as well.}
\label{tab:analysis}
\begin{tabular}{r|c|cc|cc}
  % \hline
  \toprule
  
  \multirow{2}{*}{Kernels} & 
  \multirow{2}{*}{Work (\#Flops)} & 
  \multicolumn{2}{c|}{Storage Space (\#Bytes)} & 
  \multicolumn{2}{c}{Memory Access (\#Bytes)} \\
  % \multicolumn{2}{c}{Operational Intensity (OI)} \\ 

  &
  &  
  COO &
  HiCOO &
  COO &
  HiCOO \\ \hline
  % COO &
  % HiCOO 

  \TEW & 
  $\nnz $ & 
  $48 \nnz$ & 
  $21 \nnz + 60 n_b$ &
  $36 \nnz$ &
  $18 \nnz + 40 n_b$ \\ \hline 
  % $1/36$ & 
  % $\approx 1/18$ 

  \TS & 
  $\nnz$ & 
  $32 \nnz $ &
  $40 n_b + 14 \nnz$ &
  $32 \nnz $ &
  $14 \nnz + 40 n_b$ \\ \hline
  % $1/32$ & 
  % $\approx 1/14$ \\ \hline

  \multirow{2}{*}{\TTV} & 
  \multirow{2}{*}{$2 \nnz$} & 
  $16 \nnz$ & 
  $10 \nnz + 6 \nfibs $ & 
  \multirow{2}{*}{$12 \nnz + 20 \nfibs$} &
  $12 \nnz + 8 \nfibs $ \\
  % \multirow{2}{*}{$\approx 1/6$} & 
  % \multirow{2}{*}{$\approx 1/6$} \\

  & 
  &
  $+ 12 \nfibs + 4 I$ &
  $+ 32 n_b ' + 4 I$ &
  &
  $+ 32 n_b '$ 
  \\ \hline



  \multirow{2}{*}{\TTM} & 
  \multirow{2}{*}{$2 \nnz R$} & 
  $16 \nnz + 4 \nfibs R $ & 
  $10 \nnz + 4 \nfibs R + 2 \nfibs$ & 
  $4 (\nnz + \nfibs) min\{1, \frac{R}{L}\}$ &
  $4 (\nnz + \nfibs) min\{1, \frac{R}{L}\}$ \\
  % \multirow{2}{*}{$\approx L/2$} & 
  % \multirow{2}{*}{$\approx L/2$} \\

  & 
  & 
  $+ 8 \nfibs + 4IR $ &
  $+ 32 n_b ' + 4IR$ & 
  $+ 8 \nnz + 16 \nfibs$ &
  $+ 8 \nnz + 4 \nfibs + 32 n_b '$  \\ \hline


  \multirow{2}{*}{\MTTKRP} & 
  \multirow{2}{*}{$3 \nnz R$} & 
  \multirow{2}{*}{$16 \nnz + 12 IR$} & 
  $7 \nnz + 20 n_b $ & 
  $16 \nnz $ &
  $7 \nnz + 32 n_b $ \\
  % \multirow{2}{*}{$\approx 3L/8$} &
  % \multirow{2}{*}{$\approx 3L/8$} \\

  & 
  & 
  & 
  $+ 12 IR$ & 
  $+ (8 \nnz + 4I) min\{1, \frac{R}{L}\}$ &
  $+ (8 \nnz + 4 n_b I_b) min\{1, \frac{R}{L}\}$ 
  \\

  \bottomrule
\end{tabular}
\\ $^*$ \footnotesize{Cache effect is considered only for continuous memory access in algorithms.}
}
% \\ $^1$ {\MTTKRP}s in all tensor modes can use less CSF representations than tensor order or even only one CSF representation with performance payoff.
\end{table*}



==> src/tabs/tab-kernels.tex <==
\begin{table*}[ht!]
\footnotesize
\centering
{
\caption{Sparse tensor benchmarks.}
\begin{tabular}{rp{1.5cm}p{4.5cm}p{9cm}}
  \toprule
  
  \textbf{Category} & 
  \textbf{Benchmark} & 
  \textbf{Application} & 
  \textbf{Description} \\ \hline

  Level-0 & 
  \TS & 
  Machine Learning, Quantum Chemistry & 
  Tensor-Scalar Operations \\ \hline

  Level-1 & 
  \TTV & 
  Machine Learning & 
  Tensor-Times-Vector \\ \hline

  \multirow{3}{*}{Level-2} & 
  \TTM & 
  Machine Learning, Social Network Analysis, Recommendation Systems, Quantum Chemistry, Personalized Web Search, Direct Numerical Simulation, Power Grid & 
  Tensor-Times-Matrix \\

   & 
  \MTTKRP & 
  Machine Learning, Healthcare Analytics, Quantum Chemistry, Brain Signal Analysis, Personalized Web Search, Recommendation Systems, Signal Processing, Power Grid & 
  Matriced Tensor-Times-Khatri-Rao Product \\ \hline

  %  & 
  % {\TTM}c & 
  % Machine Learning, Social Network Analysis, Quantum Chemistry, Personalized Web Search, Recommendation Systems, Direct Numerical Simulation, Power Grid & 
  % \TTM-chain \\ \hline

  \multirow{2}{*}{Level-3} & 
  \TEW & 
  Quantum Chemistry & 
  Tensor Element-Wise Operations \\

   & 
  \TTT & 
  Machine Learning, Quantum Chemistry &
  Tensor-Times-Tensor (also Tensor Contraction) \\ \hline


  \bottomrule
\end{tabular}
}
\end{table*}



==> src/tabs/tab-storage.tex <==
\begin{table}[htbp]
\centering
\footnotesize
{
\caption{Sparse tensors memory storage.}
\label{tab:storage}
\begin{tabular}{cc}
  \begin{tabular}{rcc}
    Tensors & COO (MB) & HiCOO (MB) \\
    \toprule
    \tennm{vast} & 397 & 175 \\
    \tennm{nell2} & 1150 & 543 \\ 
    \tennm{choa} & 411 & 192 \\
    \tennm{darpa} & 434 & 307 \\ 
    \tennm{fb-m} & 1480 & 1420 \\ 
    \tennm{fb-s} & 2080 & 2110 \\
    \tennm{deli} & 2090 & 3490 \\
    \tennm{nell1} & 2140 & 3160 \\ 
    \midrule
    \tennm{crime4d} & 102 & 41 \\
    \tennm{nips4d} & 59 & 25 \\ 
    \tennm{enron4d} & 1010 & 459 \\ 
    \tennm{flickr4d} & 2100 & 1740 \\ 
    \tennm{deli4d} & 2610 & 3540 \\ 
    \bottomrule
  \end{tabular}

  \begin{tabular}{rcc}
    \multirow{2}{*}{Tensors} & \multirow{2}{*}{COO (MB)} & \multirow{2}{*}{HiCOO (MB)} \\
    & & \\
    \toprule
    \tennm{regS} & 16 & 25 \\
    \tennm{regM} & 175 & 293 \\
    \tennm{regL} & 1410 & 2380 \\
    \tennm{irrS} & 16 & 7 \\
    \tennm{irrM} & 156 & 70 \\
    \tennm{irrL} & 1260 & 584 \\
    \midrule
    \tennm{regS4d} & 19 & 25 \\
    \tennm{regM4d} & 215 & 344 \\
    \tennm{regL4d} & 2060 & 3290 \\
    \tennm{irrS4d} & 31 & 12 \\
    \tennm{irrM4d} & 373 & 149 \\
    \tennm{irrL4d} & 2030 & 833 \\
    \bottomrule
  \end{tabular}
\end{tabular}
}
\end{table}
